Seeing Through the Glass: Neural 3D Reconstruction of Object Inside a Transparent Container

In this paper, we define a new problem of recovering the 3D geometry of an object confined in a transparent enclosure. We also propose a novel method for solving this challenging problem. Transparent enclosures pose challenges of multiple light reflections and refractions at the interface between different propagation media e.g. air or glass. These multiple reflections and refractions cause serious image distortions which invalidate the single viewpoint assumption. Hence the 3D geometry of such objects cannot be reliably reconstructed using existing methods, such as traditional structure from motion or modern neural reconstruction methods. We solve this problem by explicitly modeling the scene as two distinct sub-spaces, inside and outside the transparent enclosure. We use an existing neural reconstruction method (NeuS) that implicitly represents the geometry and appearance of the inner subspace. In order to account for complex light interactions, we develop a hybrid rendering strategy that combines volume rendering with ray tracing. We then recover the underlying geometry and appearance of the model by minimizing the difference between the real and hybrid rendered images. We evaluate our method on both synthetic and real data. Experiment results show that our method outperforms the state-of-the-art (SOTA) methods. Codes and data will be available at https://github.com/hirotong/ReNeuS

==> fig/ablation_depth.tex <==
\begin{figure}[htb]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/ablation_depth.pdf}
    \caption{We evaluate the performance of ReNeuS at different tracing depth. Our method generally performs better with deeper ray tracing depth showing that the proposed hybrid rendering strategy models the scene well.}
    \label{fig:ablation_depth}
\end{figure}

==> fig/calibration.tex <==
\begin{figure}[ht!]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{0.95\linewidth}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/calibration/0012.png}
    \caption{Capture set-up.}
    \label{fig:calibration_a}
    \end{subfigure}
\begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/calibration/line_image.jpg}
    \caption{Edges.}
    \label{fig:calibration_b}
\end{subfigure}\hfill
\begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/calibration/intersection.png}
    \caption{Intersections.}
    \label{fig:calibration_c}
\end{subfigure}\hfill
\begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/calibration/box.jpg}
    \caption{Box geometry.}
    \label{fig:calibration_d}
\end{subfigure}
\begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/calibration/crop.png}
    \caption{Cropped image.}
    \label{fig:calibration_e}
\end{subfigure}
    \end{minipage}
    \caption{Process of real dataset calibration. (a) Data capture equipment. (b) Labeled edges of the box. (c) Intersections of the edges. (d) Calibrated geometry of the box. (e) Cropped image and box mask.}
    \label{fig:calibration}
\end{figure}

==> fig/chart_sup.tex <==
\begin{figure}[h]
\setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/ablation_transloss.pdf}
    \caption{We show the influence of transmittance loss. Results show that the loss can promote the effectiveness of ReNeuS and we find $\lambda_1 = 0.1$ to be a balance between sparsity and reconstruction quality on the proposed dataset.}
    \label{fig:ablation_transloss}
\end{figure}

==> fig/dataset.tex <==
\begin{figure*}[ht]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{1\linewidth}%\vspace{-8em}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{beetle}}
    \begin{minipage}{0.16\linewidth}
        \centerline{\small \textbf{w/box}}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
    \centerline{\small \textbf{w/o box}}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_wobox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
    \centerline{\small \textbf{w/box}}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
    \centerline{\small \textbf{w/o box}}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_wobox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
    \centerline{\small \textbf{w/box}}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
    \centerline{\small \textbf{w/o box}}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{box}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_withbox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_wobox_0003.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}

        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}

        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{butterfly}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{coral}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{coral2}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{dinosaur}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{goku}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_withbox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_wobox_0003.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \end{minipage}
    \end{figure*}
    \begin{figure*}[t!]\ContinuedFloat\vspace{-3em}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{insect}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{insect2}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_withbox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_wobox_0003.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{lobster}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_withbox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_wobox_0003.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}

        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{shiba}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{statuette}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_withbox_0003.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_wobox_0003.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{vase}}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_withbox_0000.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_wobox_0000.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_withbox_0001.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_wobox_0001.png}
    \end{minipage}
        \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_withbox_0002.png}
    \end{minipage}
    \begin{minipage}{0.16\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_wobox_0002.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \caption{Examples of synthetic dataset.}
    \label{fig:dataset_synthetic}
\end{figure*}



==> fig/dataset_real.tex <==
\begin{figure*}[ht]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{0.9\linewidth}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample01}}\hfill
    \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample01_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample01_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample01_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample01_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample01_0004.png}
    \end{minipage}
    \end{subfigure}\vspace{0.4em}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample02}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample02_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample02_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample02_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample02_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample02_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample03}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample03_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample03_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample03_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample03_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample03_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample04}}\hfill
    \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample04_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample04_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample04_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample04_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample04_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample05}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample05_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample05_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample05_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample05_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample05_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample06}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample06_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample06_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample06_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample06_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample06_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample07}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample07_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample07_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample07_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample07_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample07_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample08}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample08_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample08_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample08_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample08_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample08_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample09}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample09_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample09_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample09_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample09_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample09_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}\vspace{-0.6em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample10}}\hfill
        \centering
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample10_0000.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample10_0001.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample10_0002.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample10_0003.png}
    \end{minipage}\hfill
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=\linewidth, height=0.7\linewidth]{fig/dataset_real/sample10_0004.png}
    \end{minipage}
    \caption*{}
    \end{subfigure}
    \end{minipage}
    \caption{Examples of real dataset}
    \label{fig:dataset_real}
\end{figure*}



==> fig/post_process.tex <==
\begin{figure}[h]
\setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{0.9\linewidth}
    \centering
    \begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/post_process/new_render_0029.jpg}
    \caption{Before process.}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/post_process/new_post_render_0029.jpg}
    \caption{After process.}
    \end{subfigure}
    \end{minipage}
    \caption{Example of mesh post-processing. We only remove the trivial facets without any further modificaiton.}
    \label{fig:post_process}
\end{figure}

==> fig/qualitative_sup.tex <==
% \begin{figure*}[ht]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
%     \centering
%     \begin{minipage}{1\linewidth}%\vspace{-8em}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{beetle}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%     \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_wobox_0000.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%     \centerline{\small \textbf{w/box}}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0003.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%     \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_wobox_0003.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%     \centerline{\small \textbf{w/box}}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%     \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{box}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_withbox_0003.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_wobox_0003.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}

%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}

%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/box_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{butterfly}}
%         \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/butterfly_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%         \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{coral}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%         \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{coral2}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/coral2_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%         \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{dinosaur}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/dinosaur_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%         \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{goku}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_withbox_0003.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_wobox_0003.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/goku_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \end{minipage}
%     \end{figure*}
%     \begin{figure*}[t!]\ContinuedFloat\vspace{-3em}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{insect}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{insect2}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_withbox_0003.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_wobox_0003.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/insect2_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%         \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{lobster}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_withbox_0003.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_wobox_0003.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%     \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/lobster_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{shiba}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/shiba_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{statuette}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_wobox_0003.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/statuette_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{1\linewidth}
%     \rotatebox[origin=c]{90}{\small \textbf{vase}}
%     \begin{minipage}{0.14\linewidth}
%         \vspace{1ex}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/beetle_withbox_0000.png}
%     \end{minipage}\hfill\vline\hfill
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_wobox_0000.png}
%     \end{minipage}
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_withbox_0001.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_wobox_0001.png}
%     \end{minipage}\hfill\vline\hfill
%         \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_withbox_0002.png}
%     \end{minipage}
%     \begin{minipage}{0.14\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/dataset/vase_wobox_0002.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \caption{Qualitative comparison.}
%     \label{fig:qualitative_sup}
% \end{figure*}

\begin{figure*}[ht]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    % \vspace{-10ex}
    \begin{minipage}{0.95\linewidth}
    \begin{subfigure}[b]{0.132\linewidth}
    \vspace{1ex}
    \begin{minipage}{1\linewidth}
        \centering
        \rotatebox{90}{\textbf{\small ~~~~~~~beetle}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/beetle_withbox_render_0001.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~~~box}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/box_withbox_render_0002.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~butterfly}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/butterfly_withbox_render_0001.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~coral}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/coral_withbox_render_0002.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~coral2}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/coral2_withbox_render_0001.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~dinosaur}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/dinosaur_withbox_render_0002.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~~goku}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/goku_withbox_render_0002.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~insect}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/insect_withbox_render_0000.png}\vspace{2ex}
        \centerline{\small GT view}
    \end{minipage}
    \caption*{}
    \end{subfigure}\hspace{1.5em}\vline\hfill
    \begin{subfigure}[b]{0.40\linewidth}
    \centering 
    \centerline{\small \textbf{w/o box}}
    \vspace{1ex}
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/beetle_wobox_colmap_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/box_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/butterfly_wobox_colmap_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral2_wobox_colmap_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/dinosaur_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/goku_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect_wobox_colmap_render_0000.jpg}\vspace{2ex}
        \centerline{\small COLMAP}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/beetle_wobox_idr_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/box_wobox_idr_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/butterfly_wobox_idr_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral_wobox_idr_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral2_wobox_idr_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/dinosaur_wobox_idr_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/goku_wobox_idr_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect_wobox_idr_render_0000.jpg}\vspace{2ex}
        \centerline{\small IDR}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/beetle_wobox_neus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/box_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/butterfly_wobox_neus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral2_wobox_neus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/dinosaur_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/goku_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect_wobox_neus_render_0000.jpg}\vspace{2ex}
        \centerline{\small NeuS}
    \end{minipage}
    \caption*{}
    \end{subfigure}\hfill\vline\hfill
    \begin{subfigure}[b]{0.40\linewidth}
    \centering
    \centerline{\small \textbf{w/box}}
    \vspace{1ex}
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/beetle_withbox_colmap_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/box_withbox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/butterfly_withbox_colmap_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral_withbox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral2_withbox_colmap_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/dinosaur_withbox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/goku_withbox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect_withbox_colmap_render_0000.jpg}\vspace{2ex}
        \centerline{\small COLMAP}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/beetle_withbox_neus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/box_withbox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/butterfly_withbox_neus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral_withbox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral2_withbox_neus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/dinosaur_withbox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/goku_withbox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect_withbox_neus_render_0000.jpg}\vspace{2ex}
        \centerline{\small NeuS}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/beetle_withbox_reneus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/box_withbox_reneus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/butterfly_withbox_reneus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral_withbox_reneus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/coral2_withbox_reneus_render_0001.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/dinosaur_withbox_reneus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/goku_withbox_reneus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect_withbox_reneus_render_0000.jpg}\vspace{2ex}
        \centerline{\small \textbf{Ours}}
    \end{minipage}%
        % \centerline{\small GT view}
    \caption*{}
    \end{subfigure}
    \end{minipage}
\end{figure*}
\begin{figure*}[t!]\ContinuedFloat
% \setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{0.95\linewidth}
    \begin{subfigure}[b]{0.132\linewidth}
    \vspace{1ex}
    \begin{minipage}{1\linewidth}
        \centering
        \rotatebox{90}{\textbf{\small ~~~~~~~insect2}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/insect2_withbox_render_0002.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~lobster}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/lobster_withbox_render_0000.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~~shiba}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/shiba_withbox_render_0002.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~statuette}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/statuette2_withbox_render_0000.png}\vspace{2ex}
        \rotatebox{90}{\textbf{\small ~~~~~~~~~vase}}%
        \includegraphics[width=1\linewidth, height=1\linewidth]{fig/qualitative_sup/vase_withbox_render_0001.png}\vspace{2ex}
        \centerline{\small GT view}
    \end{minipage}
    \caption*{}
    \end{subfigure}\hspace{1.5em}\vline\hfill
    \begin{subfigure}[b]{0.40\linewidth}
    \centering \small \textbf{w/o box}
    \vspace{1ex}
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect2_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/lobster_wobox_colmap_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/shiba_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/statuette2_wobox_colmap_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/vase_wobox_colmap_render_0001.jpg}\vspace{2ex}
        \centerline{\small COLMAP}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect2_wobox_idr_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/lobster_wobox_idr_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/shiba_wobox_idr_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/statuette2_wobox_idr_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/vase_wobox_idr_render_0001.jpg}\vspace{2ex}
        \centerline{\small IDR}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect2_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/lobster_wobox_neus_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/shiba_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/statuette2_wobox_neus_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/vase_wobox_neus_render_0001.jpg}\vspace{2ex}
        \centerline{\small NeuS}
    \end{minipage}
    \caption*{}
    \end{subfigure}\hfill\vline\hfill
    \begin{subfigure}[b]{0.40\linewidth}
    \centering \small \textbf{w/box}
    \vspace{1ex}
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect2_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/lobster_wobox_colmap_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/shiba_wobox_colmap_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/statuette2_wobox_colmap_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/vase_wobox_colmap_render_0001.jpg}\vspace{2ex}
        \centerline{\small COLMAP}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect2_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/lobster_wobox_neus_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/shiba_wobox_neus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/statuette2_wobox_neus_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/vase_wobox_neus_render_0001.jpg}\vspace{2ex}
        \centerline{\small NeuS}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/insect2_wobox_reneus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/lobster_wobox_reneus_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/shiba_wobox_reneus_render_0002.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/statuette2_wobox_reneus_render_0000.jpg}\vspace{2ex}
        \includegraphics[width=\linewidth, height=\linewidth]{fig/qualitative_sup/vase_wobox_reneus_render_0001.jpg}\vspace{2ex}
        \centerline{\small \textbf{Ours}}
    \end{minipage}%
        % \centerline{\small GT view}
    \caption*{}
    \end{subfigure}
    \end{minipage}
    \caption{Qualitative comparison on synthetic dataset.}
    \label{fig:qualitative_sup}
\end{figure*}

==> fig/real_sup.tex <==
\begin{figure*}[h]
\setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{0.95\linewidth}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample01}}\hfill
    \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample01color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample01_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample01_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample01_new.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample02}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample02color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample02_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample02_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample02_reneus.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample03}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample03color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample03_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample03_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample03_reneus.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample04}}\hfill
    \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample04color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample04_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample04_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample04_new.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample05}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample05color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample05_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample05_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample05_new.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample06}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample06color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample06_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample06_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample06_new.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample07}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample07color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample07_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample07_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample07_reneus.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample08}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample08color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample08_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample08_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample08_reneus.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample09}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample09color.JPG}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample09_colmap.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample09_neus.png}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample09_reneus.png}
    \end{minipage}
    \end{subfigure}\vspace{-0.5em}
        \centering
    \begin{subfigure}[b]{1\linewidth}
    \rotatebox[origin=c]{90}{\small \textbf{sample10}}\hfill
        \centering
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real/sample10color.JPG}
        \centerline{\small Reference}
    \end{minipage}\hfill\vline\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample10_colmap.png}
        \centerline{\small COLMAP}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample10_neus.png}
        \centerline{\small NeuS}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=\linewidth, height=0.58\linewidth]{fig/real_new/sample10_reneus.png}
        \centerline{\small \textbf{Ours}}
    \end{minipage}
    \end{subfigure}
    \end{minipage}
    \caption{Qualitative comparison on real dataset.}
    \label{fig:qualitative_real_sup}
\end{figure*}



==> fig/rebuttal.tex <==
% \begin{figure*}[ht]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
%     \centering
%     \begin{minipage}{0.95\linewidth}
%     \centering
%     \begin{subfigure}[b]{0.19\linewidth}
%     \begin{minipage}{1\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample01color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample01.png}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample06color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample06.png}
%         % \centerline{\small GT view}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}\vspace{2pt}\vline\vspace{2pt}
%     \begin{subfigure}[b]{0.19\linewidth}
%     \begin{minipage}{1\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample02color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample02.png}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample07color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample07.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}\vspace{2pt}\vline\vspace{2pt}
%         \begin{subfigure}[b]{0.19\linewidth}
%     \begin{minipage}{1\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample03color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample03.png}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample08color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample08.png}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}\vspace{2pt}\vline\vspace{2pt}
%         \begin{subfigure}[b]{0.19\linewidth}
%     \begin{minipage}{1\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample04color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample04.png}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample09color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample09.png}
%         % \centerline{\small $\text{COLMAP}_{\xi=0}$}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}\vspace{2pt}\vline\vspace{2pt}
%         \begin{subfigure}[b]{0.19\linewidth}
%     \begin{minipage}{1\linewidth}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample05color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample05.png}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample10color.JPG}
%         \includegraphics[width=\linewidth, height=\linewidth]{fig/real/sample10.png}
%         % \centerline{\small $\text{COLMAP}_{\xi=0}$}
%     \end{minipage}
%     \caption*{}
%     \end{subfigure}
%     \end{minipage}
%     \caption{Localization results visualization. The correlation results (vehicle location possibility maps) are overlayed on the satellite images}.
%     \label{fig:qualitative_real}
% \end{figure*}

\begin{figure}[t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{minipage}{0.95\linewidth}
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \begin{minipage}{1\linewidth}
        \includegraphics[width=\linewidth, height=0.9\linewidth]{fig/rebuttal/beetle_withbox_render_0006.png}
        \includegraphics[width=\linewidth, height=0.9\linewidth]{fig/rebuttal/beetle_withbox_reneus_render_0006.jpg}
        % \includegraphics[width=\linewidth, height=\linewidth]{fig/real/colmap_new.png}
    \end{minipage}
    % \centerline{\small Reference}
    \caption*{}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \begin{minipage}{1\linewidth}
        \includegraphics[width=\linewidth, height=0.9\linewidth]{fig/rebuttal/box_withbox_render_0006.png}        
        \includegraphics[width=\linewidth, height=0.9\linewidth]{fig/rebuttal/box_withbox_reneus_render_0006.jpg}    
    \end{minipage}
    % \centerline{\small Results}
    \caption*{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \begin{minipage}{1\linewidth}
        \includegraphics[width=\linewidth, height=0.9\linewidth]{fig/rebuttal/goku_withbox_render_0010.png}        
        \includegraphics[width=\linewidth, height=0.9\linewidth]{fig/rebuttal/goku_withbox_reneus_render_0010.jpg}    
    \end{minipage}
    % \centerline{\small Results}
    \caption*{}
    \end{subfigure}
    \end{minipage}
    \vspace{-1em}
    \caption{Results of ReNeuS on various shaped containers.}
    \vspace{-1.2em}
    \label{fig:rebuttal}
\end{figure}


==> others.tex <==
age intensity. A more physically correct model should be
bp = f(c
′
p ∗ h), where c
′
indicates the scene irradiance
and f(·) is the camera response function (CRF) that maps
the scene irradiance to image intensity. A nonlinear CRF
will increase the complexity of the blur kernel and make
the learning of DSK difficult if the linear model in Eq. (4) is
used, especially in high contrast regions [46]. To compensate for the nonlinear CRF, we assume that our sharp NeRF
predicts colors in linear space and adopt a simple gamma
correction function in the final output:
 \mathbf {b}_\mathbf {p} = g(\sum _{\mathbf {q}\in \mathcal {N}(\mathbf {p})} w_\mathbf {q} \mathbf {c}'_\mathbf {q}), \label {eq:gamma+spasekernel} (7)
where g(c
′
) = c
′
1
2.2 is the gamma correction function.
More complex CRFs could be used to model real world
cameras, such as pre-calibrated CRFs, or jointly optimizing
the CRFs during training. But we find this simple scheme is
enough to compensate the nonlinearity in the imaging process and improve the quality. More discussions about modeling the CRF can be found in supplementary material.


==> tables/ablation.tex <==
\begin{table}[bt]
	\begin{center}

	
	%  \makebox[\textwidth][l]{
	    \begin{tabular}{llccr}
    		\toprule   
    		    
    	    \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\small$Items$}}  &\multirow{2}{*}{\raisebox{-\heavyrulewidth}{\small{$Baseline$}}}   &\multirow{2}{*}{\raisebox{-\heavyrulewidth}{\small{$Baseline$}}}
    	    &\multirow{2}{*}{\raisebox{-\heavyrulewidth}{\small{$Baseline$}}} &\multirow{2}{*}{\raisebox{-\heavyrulewidth}{\small{$ReNeuS$}}}\\
\vspace{-0.95pt}\\
 & $ $ & $w \ refrac.$ &\small{$  tr. \ loss $}&$(ours)$\\ 
\cmidrule{1-5}




\multirow{1}{*}{Beetle}
&$NA$&$63.55$&$1.39$&$1.40$
\\
 \multirow{1}{*}{Box}
 &$2.63$&$11.95$&$2.61$&$2.29$

 	\\
 \multirow{1}{*}{Butterfly}
  &$1.00$&$1.12$&$1.10$&$1.15$

\\
  \multirow{1}{*}{Coral2}
  & $2.25$&$2.31$&$2.52$&$2.44$
 
  \\
   \multirow{1}{*}{Coral}
    &$12.33$&$14.43$&$NA$&$8.78$
   \\
  \multirow{1}{*}{Dinosaur}
  &$NA$&$NA$&$NA$&$1.47$
  \\
    \multirow{1}{*}{Goku}
    &$1.31$&$NA$&$1.47$&$1.48$
    \\
   
    \multirow{1}{*}{Insect}
    &$NA$&$1.10$&$NA$&$1.10$


    \\
    
    \multirow{1}{*}{Insect2}
    &$NA$&$1.28$&$1.27$&$1.30$
    \\
    \multirow{1}{*}{Lobster}
    &$6.36$&$12.55$&$6.29$&$11.08$
    \\
   
    \multirow{1}{*}{Shiba}
    &$3.27$&$3.37$&$3.37$&$3.38$
    \\
    \multirow{1}{*}{Statuette2}
    &$2.13$&$70.56$&$2.25$&$2.26$
%   \\
% \multirow{1}{*}{Statuette}
% &$2.67$&$2.81$&$2.77$&$2.81$
 \\
\multirow{1}{*}{Vase}
&$3.73$&$67.13$&$3.62$&$3.68$
 \\
\cmidrule{1-5}
\multirow{1}{*}{Mean}
&$3.77$&$21.01$&$\bold{2.56}$&$3.19$

\\ \vspace{-0.75em} \\

		    \bottomrule 
	    \end{tabular}
	 %   }
	    
	\end{center}
\setlength{\abovecaptionskip}{0cm} 
\setlength{\belowcaptionskip}{0cm}
\caption{Write suitable caption}
\label{tab:ablation}
\end{table}

==> tables/bsdf.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
         Parameter & Specular & Roughness & Sheen Tint & IOR & Transmission \\
         \midrule
         Value & $0.5$ & $0.05$ & $0.5$ & $1.45$ & $1.0$ \\
         \bottomrule
    \end{tabular}
    }
    \caption{Main parameters of the transparent material.}
    \label{tab:bsdf}
\end{table}

==> tables/dataset.tex <==
\begin{table}[ht]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
        \toprule
         Dataset & $N_{obj}$ & $N_{view}$ & Resolution & Mask & Camera pose & GT model \\
        \midrule
         w/box & 13 & 60 & $800 \times 800$ & box & GT & True \\
         w/o box & 13 & 60 & $800 \times 800$ & object & GT & True \\
         real & 10 & 60 & $1728 \times 1152$ & box & estimated &False \\
         \bottomrule
    \end{tabular}
    }
    \caption{Summary of the proposed dataset.}
    \label{tab:dataset}
\end{table}

==> tables/license.tex <==
\begin{table*}[ht]
    \centering
    \renewcommand\arraystretch{0.85}
    \resizebox{0.95\linewidth}{!}{
    % \setlength{\tabcolsep}{5mm}
    
    \begin{tabular}{lll}
    \toprule
        Item & License & \textbf{URL} \\
        \hline
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/eastern-hercules-beetle-a6f2a6fe7a3c4d19831f1bd79d664dcc}{beetle}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/eastern-hercules-beetle-a6f2a6fe7a3c4d19831f1bd79d664dcc}}\\
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/tollkiste-00fa12d17fe04dc39e9275164f5339c1}{box}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/tollkiste-00fa12d17fe04dc39e9275164f5339c1}} \\
         & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/common-lime-butterfly-smoothie-3d-078da6e1f86c4d2ca874e3f4381becb8}{butterfly}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/common-lime-butterfly-smoothie-3d-078da6e1f86c4d2ca874e3f4381becb8}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/pocillopora-eydouxi-b2a7aef9f4814de09d42546c1a974cd0}{coral}} & \multirow{2}{3cm}{\small CC BY-NC-SA 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/pocillopora-eydouxi-b2a7aef9f4814de09d42546c1a974cd0}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/pocillopora-meandrina-3bacf518167b46d78fef48ef9e0b7019}{coral2}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/pocillopora-meandrina-3bacf518167b46d78fef48ef9e0b7019}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/squelette-entier-de-felin-espece-inconnue-9b7ae513a2294711a9e083de1a4dcae5}{dinosaur}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/squelette-entier-de-felin-espece-inconnue-9b7ae513a2294711a9e083de1a4dcae5}}\\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/goku-3d-scan-dragon-ball-3db326f4b41f4a00bbd116fad7f4d09e}{goku}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/goku-3d-scan-dragon-ball-3db326f4b41f4a00bbd116fad7f4d09e}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/cicindela-campestris-b13a625c2e3b4b6aa26a27711a0cac39}{insect}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/cicindela-campestris-b13a625c2e3b4b6aa26a27711a0cac39}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/prosopocoilus-savagei-b04ad901d4344ccf8ec6893a6b36c27c}{insect2}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/prosopocoilus-savagei-b04ad901d4344ccf8ec6893a6b36c27c}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/panulirus-longipes-d7cc2b585ad943ef81274e014e6f745b}{lobster}} & \multirow{2}{3cm}{CC0 1.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/panulirus-longipes-d7cc2b585ad943ef81274e014e6f745b}} \\ & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/free-toon-shiba-inu-3d-model-ae0a62c3d588496fa9d5e516fcb6786c}{shiba}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/free-toon-shiba-inu-3d-model-ae0a62c3d588496fa9d5e516fcb6786c}} \\ 
        & & \\
        \multirow{2}{1.5cm}{\href{https://www.turbosquid.com/3d-models/3d-statuette-sheep-barrel-model-1335035}{statuette}} & \multirow{2}{3cm}{TurboSquid standard} & \multirow{2}{13cm}{\url{https://www.turbosquid.com/3d-models/3d-statuette-sheep-barrel-model-1335035}} \\
        & & \\
        \multirow{2}{1.5cm}{\href{https://sketchfab.com/3d-models/vase-951156fb0db74176af08501bdb4b5acd}{vase}} & \multirow{2}{3cm}{CC BY 4.0} & \multirow{2}{13cm}{\url{https://sketchfab.com/3d-models/vase-951156fb0db74176af08501bdb4b5acd}} \\ 
        & & \\
        \bottomrule
    \end{tabular}
    }
    \caption{Dataset source and license information.}
    \label{tab:license}
\end{table*}





==> tables/without_box.tex <==
\begin{table}[bt]
	\begin{center}

	
	  \makebox[\textwidth][l]{
	    \begin{tabular}{ll|c|c|c|c}
    		\toprule   
    		    
    	    \multirow{2}{*}{\raisebox{-\heavyrulewidth}{$Items$}} & \multicolumn{2}{c|}{\raisebox{-\heavyrulewidth}{\small{$COLMAP$}}}  & \multirow{2}{*}{\small{$IDR$}}&\multirow{2}{*}{\small{$NeuS$}} &\multirow{2}{*}{\small{$ReNeuS$}}\\
\cmidrule{2-3}
 & \small{trim $0$} & \small{trim $7$} &$ $&$ $&$(ours)$\\ 
\cmidrule{1-6}

\multirow{2}{*}{beetle}
	&$15.48$	&$17.55$	&$-$	&$27.40$ &$xx$\\
  &$1.10$	&$3.67$	&$0.76$	&$2.42$ &$-$
 \\ \vspace{-0.75em} \\
 \multirow{2}{*}{box} 
 	&$35.38$	&$14.15$	&$-$	&$15.43$	&$5.46$
  \\
 
  &$4.09$	&$5.28$	&$0.51$	&$3.76$&$-$
 \\ \vspace{-0.75em} \\
 \multirow{2}{*}{butterfly}
 %\lightrulewidth
 &$12.44$	&$18.82$	&$-$	&$19.85$	&$1.73$ \\
  &$6.10$	&$1.15$	&$0.78$	&$9.98$&$-$
 \\ \vspace{-0.75em} \\
  \multirow{2}{*}{coral2}
  &$21.38$	&$29.25$	&$-$	&$20.75$	&$3.91$
  \\
  &$1.81$	&$2.75$	&$1.66$	&$1.42$&$-$
 \\ \vspace{-0.75em} \\
   \multirow{2}{*}{coral}
   &$142$	&$17.32$	&$-$	&$21.18$
  \\
  &$4.93$	&$11.23$	&$1.68$	&$2.11$&$-$
  \\ \vspace{-0.75em} \\
  \multirow{2}{*}{dinosaur}
  	&$28.15$	&$36.33$	&$-$	&$15.46$	&$1.51$
    \\
    &$2.22$	&$1.18$	&$0.82$	&$2.80$&$-$
    \\ \vspace{-0.75em} \\
    \multirow{2}{*}{goko}
    &$22.48$	&$11.09$	&$-$	&$17.23$
    \\
    &$2.21$	&$2.13$	&$0.81$	&$1.37$&$-$
   \\ \vspace{-0.75em} \\
    \multirow{2}{*}{insect}
    &$45.78$	&$35.88$	&$-$	&$21.71$
    \\
    &$2.56$	&$0.96$	&$0.62$	&$5.89$&$-$
    \\ \vspace{-0.75em} \\
    \multirow{2}{*}{insect2}
    &$15.34$	&$18.65$	&$-$	&$22.11$
    \\
    &$1.34$	&$1.15$	&$0.76$&$4.07$&$-$
   \\ \vspace{-0.75em} \\
    \multirow{2}{*}{lobster}
    &$40.52$	 	&$26.72$	&$-$ &$14.61$
    \\
    &$13.27$	&$12.20$	&$17.17$	&$12.97$&$-$
   \\ \vspace{-0.75em} \\
    \multirow{2}{*}{shiba}
    &$24.30$	&$13.92$	&$-$	&$20.30$
    
    \\
    &$2.33$	&$17.73$	&$2.24$	&$2.22$&$-$
   \\ \vspace{-0.75em} \\
    \multirow{2}{*}{statuette2}
    &$61.74$	&$22.16$	&$-$	&$25.44$ 

\\
&$0.85$	&$0.92$	&$0.87$	&$0.79$	&$-$
\\ \vspace{-0.75em} \\
 \multirow{2}{*}{statuette}
 &$21.55$	&$15.71$	&$-$	&$22.17$	\\
 &$0.98$	&$1.00$	&$1.93$	&$0.96$	&$-$
 \\ \vspace{-0.75em} \\
\multirow{2}{*}{vase}
&$15.02$	&$15.06$	&$-$	&$24.68$

\\
&$1.37$	&$1.30$	&$1.31$	&$1.35$	&$-$
\\ \vspace{-0.75em} \\
\multirow{2}{*}{mean}
&$35.86$	&$20.83$	&$\#DIV/0! $	&$20.59$	&$3.15$\\
	&$3.22$	&$4.47$	&$2.28$	&$3.72$&$-$
\\ \vspace{-0.75em} \\

		    \bottomrule 
	    \end{tabular}
	    }
	    
	\end{center}
\setlength{\abovecaptionskip}{0cm} 
\setlength{\belowcaptionskip}{0cm}
\caption{Write suitable caption}
\label{tab:without_box}
\end{table}
